Learning Causal Domain-Invariant Temporal Dynamics for Few-Shot Action Recognition

Few-shot action recognition aims at quickly adapting a pre-trained model to the novel data with a distribution shift using only a limited number of samples. Key challenges include how to identify and leverage the transferable knowledge learned by the pre-trained model. We therefore propose CDTD, or Causal Domain-Invariant Temporal Dynamics for knowledge transfer. To identify the temporally invariant and variant representations, we employ the causal representation learning methods for unsupervised pertaining, and then tune the classifier with supervisions in next stage. Specifically, we assume the domain information can be well estimated and the pre-trained image decoder and transition models can be well transferred. During adaptation, we fix the transferable temporal dynamics and update the image encoder and domain estimator. The efficacy of our approach is revealed by the superior accuracy of CDTD over leading alternatives across standard few-shot action recognition datasets.

==> algo/algo.tex <==
\begin{algorithm}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{\ourmeos}
	\label{alg1}
	\begin{algorithmic}[h]
    % \hline
    \textbf{Training on the base data}
    \hline
        \REQUIRE video sequence $\rvv_k$, there exists $i$ clips for each video sequence
        \STATE Initialization: perception$\{g_\omega\}$, invariant transition $\{f_\phi\}$, variant transition $\{f_\theta\}$
        % \STATE \algorithmicwhile \HS not done
        \WHILE{ not done} 
        \FOR{\HS$i=1,2,...$} 
		\STATE $\theta\leftarrow\theta-\frac{\partial \mathcal{L}^i_{\text{ELBO}}}{\partial\theta}$
		\ENDFOR
        \STATE Update $\omega\leftarrow\omega-\frac{\partial \mathcal{L}^k_{\text{ELBO}}}{\partial \omega}$ 
        \STATE Update $\phi\leftarrow\phi-\frac{\partial \mathcal{L}^k_{\text{ELBO}}}{\partial\phi}$
        \ENDWHILE
        \STATE Update $\psi\leftarrow\psi-\frac{\partial \mathcal{L}^k_{\text{cls}}}{\partial\psi}$
		\ENSURE $\{\omega,\phi,\theta, \psi\}$. 
        \vspace{0.2cm}
        \hline
        \vspace{0.1cm}
        \textbf{Adapting to the novel data}
        \vspace{0.1cm}
        \hline
        \REQUIRE video sequence $\rvv_k$
        \STATE $\{\omega,\phi,\theta, \psi\}$ learned from the base data
        % \STATE \algorithmicwhile \HS not done
        \WHILE{ not done} 
        \FOR{\HS$i=1,2,...$} 
		\STATE $\theta'\leftarrow\theta-\frac{\partial \mathcal{L}^i_{\text{ELBO}}}{\partial\theta}$
		\ENDFOR
        \ENDWHILE
        \STATE Update $\psi'\leftarrow\psi-\frac{\partial \mathcal{L}^k_{\text{cls}}}{\partial\psi}$
		\ENSURE $\{\omega,\phi,\theta', \psi'\}$.
	\end{algorithmic}  
\end{algorithm}

==> change.tex <==
1. Figure 1: is that

==> tab/tab_allway_ssv2.tex <==
% \begin{wraptable}{r}{0.6\textwidth}
% \small
% \vspace{-0.1cm}
\begin{table}[h]
\centering
% \small
\caption{Comparing TCMT$_C$ to benchmarks for all-way-k-shot on the SSv2 dataset.}
\label{tab:allway_ssv2}
\scalebox{0.8}{
\begin{tabular}{l|c|cccc}
\hline\hline
{}
& {}
% &\multicolumn{2}{c}{Sth-Else}
&\multicolumn{4}{c}{SSv2}
\\ \hline
{}
& Backbone
% &{5-shot}
% &{10-shot}
&{2-shot}
&{4-shot}
&{8-shot}
&{16-shot}
\\ \hline 
ActionCLIP & ViT-B/16 & 4.1 & 5.8 & 8.4 & 11.1 \\
XCLIP    & ViT-B/16  & 3.9 & 4.5 & 6.8 & 10.0  \\
XFLORENCE  & ViT-B/16     &  4.2 & 6.1 & 7.9 & 10.4\\
VideoPrompt & ViT-B/16 & 4.4 & 5.1 & 6.1 & 9.7  \\
% BIKE  & ViT-B/16     &  \\
ViFi-CLIP  & ViT-B/16  & 6.2 & 7.4 & 8.5 & 12.4 \\
VL Prompting  & ViT-B/16  & \underline{6.7} & \underline{7.9} & \underline{10.2} & \underline{13.5} \\
\bf{TCMT$_C$} & ViT-B/16 & \bf{7.5} & \bf{9.6} & \bf{11.8} & \bf{15.5}  \\
\hline\hline
\end{tabular}
\vspace{-0.2cm}
}
\end{table}
% \end{wraptable}
